Operability timescale of defect-engineered graphene

Defects in the lattice are of primal importance to tune graphene chemical, thermal and electronic properties. Electron-beam irradiation is an easy method to induce defects in graphene following pre-designed patterns, but no systematic study of the time evolution of the resulting defects is available. In this paper, the change over time of defected sites created in graphene with low-energy ($\leq 20$ keV) electron irradiation is studied both experimentally via micro-Raman spectroscopy for a period of $6\times 10^3$ hours and through molecular dynamics simulations. During the first 10 h, the structural defects are stable at the highest density value. Subsequently, the crystal partially reconstructs, eventually reaching a stable, less defected condition after more than one month. The simulations allow the rationalization of the processes at the atomic level and confirm that the irradiation induces composite clusters of defects of different nature rather than well-defined nanoholes as in the case of high-energy electrons. The presented results identify the timescale of the defects stability, thus establishing the operability timespan of engineerable defect-rich graphene devices with applications in nanoelectronics. Moreover, long-lasting chemical reactivity of the defective graphene is pointed out. This property can be exploited to functionalize graphene for sensing and energy storage applications.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
